Mithridates: Auditing and Boosting Backdoor Resistance of Machine Learning Pipelines

Machine learning (ML) models trained on data from potentially untrusted sources are vulnerable to poisoning. A small, maliciously crafted subset of the training inputs can cause the model to learn a "backdoor" task (e.g., misclassify inputs with a certain feature) in addition to its main task. Recent research proposed many hypothetical backdoor attacks whose efficacy heavily depends on the configuration and training hyperparameters of the target model. Given the variety of potential backdoor attacks, ML engineers who are not security experts have no way to measure how vulnerable their current training pipelines are, nor do they have a practical way to compare training configurations so as to pick the more resistant ones. Deploying a defense requires evaluating and choosing from among dozens of research papers and re-engineering the training pipeline. In this paper, we aim to provide ML engineers with pragmatic tools to audit the backdoor resistance of their training pipelines and to compare different training configurations, to help choose one that best balances accuracy and security. First, we propose a universal, attack-agnostic resistance metric based on the minimum number of training inputs that must be compromised before the model learns any backdoor. Second, we design, implement, and evaluate Mithridates a multi-stage approach that integrates backdoor resistance into the training-configuration search. ML developers already rely on hyperparameter search to find configurations that maximize the model's accuracy. Mithridates extends this standard tool to balance accuracy and resistance without disruptive changes to the training pipeline. We show that hyperparameters found by Mithridates increase resistance to multiple types of backdoor attacks by 3-5x with only a slight impact on accuracy. We also discuss extensions to AutoML and federated learning.

==> usenix-2020-09 <==
% usenix.sty - to be used with latex2e for USENIX.
% To use this style file, look at the template usenix2019_v3.1.tex
%
% $Id: usenix.sty,v 1.2 2005/02/16 22:30:47 maniatis Exp $
%
% The following definitions are modifications of standard article.sty
% definitions, arranged to do a better job of matching the USENIX
% guidelines.
% It will automatically select two-column mode and the Times-Roman
% font.
%
% 2018-12-19 [for ATC'19]: add packages to help embed all fonts in
%   pdf; to improve appearance (hopefully); to make refs and citations
%   clickable in pdf
%
% 2020-09-21 file updated to comment out flushend and make it optional

%
% USENIX papers are two-column.
% Times-Roman font is nice if you can get it (requires NFSS,
% which is in latex2e.

\if@twocolumn\else\input twocolumn.sty\fi
\usepackage{mathptmx}  % times roman, including math (where possible)

% hopefully embeds all fonts in pdf
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{pslatex}

% appearance
\usepackage[kerning,spacing]{microtype} % more compact and arguably nicer

% Uncomment the following line if you want the columns of the last page 
% equal in size. But note that doing so may cause issues with some 
% document-generating tools.
% \usepackage{flushend}

% refs and bib
\usepackage{cite}               % order multiple entries in \cite{...}
\usepackage{breakurl}           % break too-long urls in refs
\usepackage{url}                % allow \url in bibtex for clickable links
\usepackage{xcolor}             % color definitions, to be use for...
\usepackage[]{hyperref}         % ...clickable refs within pdf...
\hypersetup{                    % ...like so
  colorlinks,
  linkcolor={green!80!black},
  citecolor={red!70!black},
  urlcolor={blue!70!black}
}

%
% USENIX wants margins of: 0.75" sides, 1" bottom, and 1" top.
% 0.33" gutter between columns.
% Gives active areas of 7" x 9"
%
\setlength{\textheight}{9.0in}
\setlength{\columnsep}{0.33in}
\setlength{\textwidth}{7.00in}

\setlength{\topmargin}{0.0in}

\setlength{\headheight}{0.0in}

\setlength{\headsep}{0.0in}

\addtolength{\oddsidemargin}{-0.25in}
\addtolength{\evensidemargin}{-0.25in}

% USENIX wants no page numbers for camera-ready papers, so that they can
% number them themselves.  But submitted papers should have page numbers
% for the reviewers' convenience.
% 
%
% \pagestyle{empty}

%
% USENIX titles are in 14-point bold type, with no date, and with no
% change in the empty page headers.  The whole author section is 12 point
% italic--- you must use {\rm } around the actual author names to get
% them in roman.
%
\def\maketitle{\par
 \begingroup
   \renewcommand\thefootnote{\fnsymbol{footnote}}%
   \def\@makefnmark{\hbox to\z@{$\m@th^{\@thefnmark}$\hss}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hbox to1.8em{\hss$\m@th^{\@thefnmark}$}##1}%
   \if@twocolumn
     \twocolumn[\@maketitle]%
     \else \newpage
     \global\@topnum\z@
     \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}%
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@maketitle{\newpage
 \vbox to 2.5in{
 \vspace*{\fill}
 \vskip 2em
 \begin{center}%
  {\Large\bf \@title \par}%
  \vskip 0.375in minus 0.300in
  {\large\it
   \lineskip .5em
   \begin{tabular}[t]{c}\@author
   \end{tabular}\par}%
 \end{center}%
 \par
 \vspace*{\fill}
% \vskip 1.5em
 }
}

%
% The abstract is preceded by a 12-pt bold centered heading
\def\abstract{\begin{center}%
{\large\bf \abstractname\vspace{-.5em}\vspace{\z@}}%
\end{center}}
\def\endabstract{}

%
% Main section titles are 12-pt bold.  Others can be same or smaller.
%
\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus-1ex minus
    -.2ex}{2.3ex plus.2ex}{\reset@font\large\bf}}
